A Resilience Framework for Bi-Criteria Combinatorial Optimization with Bandit Feedback

We study bi-criteria combinatorial optimization under noisy function evaluations. While resilience and black-box offline-to-online reductions have been studied in single-objective settings, extending these ideas to bi-criteria problems introduces new challenges due to the coupled degradation of approximation guarantees for objectives and constraints. We introduce a notion of $(\alpha,\beta,\delta,\texttt{N})$-resilience for bi-criteria approximation algorithms, capturing how joint approximation guarantees degrade under bounded (possibly worst-case) oracle noise, and develop a general black-box framework that converts any resilient offline algorithm into an online algorithm for bi-criteria combinatorial multi-armed bandits with bandit feedback. The resulting online guarantees achieve sublinear regret and cumulative constraint violation of order $\tilde{O}(\delta^{2/3}\texttt{N}^{1/3}T^{2/3})$ without requiring structural assumptions such as linearity, submodularity, or semi-bandit feedback on the noisy functions. We demonstrate the applicability of the framework by establishing resilience for several classical greedy algorithms in submodular optimization.

==> Experiments.tex <==

\section{Experiments}\label{sec:exp}

In this section, we empirically evaluate the $\delta$ resilience guarantees we derived and evaluate regret and cumulative constraint violations for the online bi-criteria CMAB algorithms our framework adapted from those offline algorithms. 

\subsection{Offline Problems} \label{sec:exp:offline}

\todo[inline]{Subham: after you update the experiment section with the results for bi-criteria CMAB, can you also add results for experiments in the offline setting? 

for a fixed problem and for a fixed epsilon, get "exact" query values and add/subtract epsilon (maybe bernoulli(1/2)), run the offline alg (so not using CMAB framework, just offline alg), and then evaluate the final solution, $f(S^A)$ and $g(S^A)$ (eg def 1).

maybe for each alg run, can have a plot with x-axis for $\epsilon$, y-axis for f (another plot for g), plotting both the bound we derived (RHS of (1), (2)) and the achieved value (LHS of (1), (2));  

if problem can't get OPT, then could plot horizontal line for f(GRD) (where GRD is based on exact values)) and we show how solution degrades with $\epsilon$ compared to the -$\delta$ $\epsilon$ degradation we derived.}


% \begin{figure}[h]
% % \centering
% % \includegraphics[width=8cm]{Neurips 2025/figures/bicriteria-offline-exp-plot-sketch.png}
% \centering
% \begin{minipage}{0.24\textwidth}
%   \includegraphics[width=\linewidth]{Neurips 2025/figures/result11.png}\\
%   \centering \small (a) \label{1a}
% \end{minipage}\hfill
% \begin{minipage}{0.24\textwidth}
% \includegraphics[width=\linewidth]{Neurips 2025/figures/result1.png}\\
%   \centering \small (b) \label{1b}
% \end{minipage}\hfill
% \begin{minipage}{0.24\textwidth}
% \includegraphics[width=\linewidth]{Neurips 2025/figures/result22.png}\\
%   \centering \small (c) \label{1c}
% \end{minipage}
% \hfill
%   \begin{minipage}{0.24\textwidth}
%   \includegraphics[width=\linewidth]{Neurips 2025/figures/result2.png}\\
%   \centering \small (d) \label{1d}
% \end{minipage}
% \caption{Bi-criteria resilience of \texttt{MINTSS}. Worst-case performance over various additive perturbations of maginitude $\epsilon$ for various $\epsilon$ for both objective and constraint function value queries.  Since $\mathrm{OPT}$ is unknown, $f(S^{\mathcal{A}})$ is compared against the more challenging $f(\mathcal{GRD}) - \delta \epsilon$  .
% We also report that the largest number of oracle calls observed was xxx, which is less than our bound $N=$
% \hl{update: constraint should be $+\delta\epsilon$ and go up}
% }
% \label{fig:1}
% \end{figure}


\begin{figure}[h]
% \centering
% \includegraphics[width=8cm]{Neurips 2025/figures/bicriteria-offline-exp-plot-sketch.png}
\centering
\begin{minipage}{0.24\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures2/res_1a.png}\\
  \centering \small (a) \label{1a}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
\includegraphics[width=\linewidth]{Neurips 2025/figures2/res_2a.png}\\
  \centering \small (b) \label{1b}
\end{minipage}
\hfill
\begin{minipage}{0.24\textwidth}
\includegraphics[width=\linewidth]{Neurips 2025/figures2/res_1b.png}\\
  \centering \small (c) \label{1c}
\end{minipage}\hfill
  \begin{minipage}{0.24\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures2/res_2b.png}\\
  \centering \small (d) \label{1d}
\end{minipage}
% \begin{minipage}{0.24\textwidth}
%   \includegraphics[width=\linewidth]{Neurips 2025/figures2/res_1a.png}\\
%   \centering \small (a) \label{1a}
% \end{minipage}\hfill
% \begin{minipage}{0.24\textwidth}
% \includegraphics[width=\linewidth]{Neurips 2025/figures2/res_1b.png}\\
%   \centering \small (b) \label{1b}
% \end{minipage}\hfill
% \begin{minipage}{0.24\textwidth}
% \includegraphics[width=\linewidth]{Neurips 2025/figures2/res_2a.png}\\
%   \centering \small (c) \label{1c}
% \end{minipage}
% \hfill
%   \begin{minipage}{0.24\textwidth}
%   \includegraphics[width=\linewidth]{Neurips 2025/figures2/res_2b.png}\\
%   \centering \small (d) \label{1d}
% \end{minipage}



\caption{Bi-criteria resilience of \texttt{MINTSS}. Worst-case performance over various additive perturbations of maginitude $\epsilon$ for various $\epsilon$ for both objective and constraint function value queries.  Since $\mathrm{OPT}$ is unknown, $f(S^{\mathcal{A}})$ is compared against the more challenging $f(\mathcal{GRD}) - \delta \epsilon$  .
We also report that the largest number of oracle calls observed was 39, which is less than our bound $N=n^2$.
% \hl{update: constraint should be $+\delta\epsilon$ and go up}
\\Figures (a) and (c) correspond to the setting with $\kappa = 0.98$, $\omega = 0.15$, representing a higher relaxation regime, while figures (b) and (d) correspond to $\kappa = 0.98$, $\omega = 0.08$, indicating a lower relaxation regime.
}
\label{fig:2}
\end{figure}

\paragraph{Baselines:}  Since our work is the first to derive resilience guarantees for this algorithm, we do not have alternative $\delta$ resilience bounds to compare with.  We instead use an upper bound based on exact oracles and observed empirical performance under certain perturbations (though due to the prohibitive search for worst-case perturbations, these are not necessarily worst-case perturbations).  
Following our \cref{def:robustness}, for the objective $f$ it would be natural to compare our $\alpha f(\mathrm{OPT}) 
+\delta \epsilon$ bound against observed resilience, $f(\mathrm{OPT})$ and $\alpha f(\mathrm{OPT})$.
However, except for trivial cases, identifying $\mathrm{OPT}$ is prohibitive.  
We instead compare against observed resilience $f(\mathrm{S^\mathcal{A}})$ over different $\epsilon$, and $f(\mathrm{S^\mathcal{A}_{\epsilon=0}})$, where $\mathrm{S^\mathcal{A}_{\epsilon=0}}$ denotes the algorithm $\mathcal{A}$ run with access to exact oracles.  
Since the algorithm is deterministic, we do not take an expectation.
For the constraint $g$, we can evaluate $\beta \kappa$, though we likewise instead use the tighter $\mathrm{g^\mathcal{A}_{\epsilon=0}}$ and examine the degradation with respect to $\epsilon$ due to inexact oracles.

To empirically evaluate resilience for a specific $\epsilon$, we run algorithm $\mathcal{A}$ using i.i.d.~random value perturbations of the form $\hat{f}(S) \gets f(S) + (-1)^{\mathrm{Be}(p)}$ and $\hat{g}(S) \gets g(S) + (-1)^{\mathrm{Be}(p)}$ for different probabilities $p$.  
We fix $p\in\{0, \frac{1}{4}, \frac{1}{2}, \frac{3}{4},1\}$, and for $0<p<1$ we conduct 10 runs, taking the worst case $f(\mathrm{S^\mathcal{A}})$ and the worst case $g(\mathrm{S^\mathcal{A}})$ over the runs. 
We note that this procedure does not (necessarily) yield a worst-case sequence of perturbations for $\mathcal{A}$, 
so a large gap between our bound and the empirically observed resilience is not dispositive that our derived $\delta$ is loose. % (possibly from different trials).
Lastly, we also record the worst-case number for oracle calls over all runs (any $\epsilon$) and compare to our bound $\texttt{N}$.


\paragraph{Implementation Details:}
In the experimental setting, we consider 20 nodes (arms) divided into 4 groups with group sizes $[6, 6, 6, 2]$, corresponding utilities $[0.1,0.2,0.3,0.4]$, and costs for each node are $\frac{1}{20}$, respectively. This forms a weighted cover problem.

We implement the offline MINTSS algorithm for the monotone cost submodular cover problem and evaluate its resilience to $\epsilon$-noise. Node selection is based on marginal gain, but the utility oracle $g(S^\mathcal{A}_{\epsilon=p})$ introduces noise, misreporting $-\epsilon$ with probability $p$. The stopping criterion is defined as the minimum cost subset such that the utility threshold is met i.e.$g(S^\mathcal{A}_{\epsilon=p}) \geq \kappa - \omega$.

When the algorithm selects a subset for the \texttt{submodular set cover problem} based on the noisy oracle $g(S^\mathcal{A})$, the utility is normalized by a constant factor to ensure the sum of rewards of the selected set is scaled appropriately. Due to underreporting with noisy oracle call, the utility underestimation propagates as additive $+\epsilon$ cost in $f(S^\mathcal{A})$, potentially exceeding/overestimating $f(\mathcal{GRD})$ if greedy is optimal, or $f(\mathrm{OPT})$ otherwise. This leads to additive noise in the monotone cost in the noiseless cost function $f(S^\mathcal{A})$.



\paragraph{Observations on Offline Noise-Oracular Impact on Cost and Utility}

The maximum number of noisy oracle calls is reported as $N = [22, 23, 27, 39, 39, 39]$ corresponding to $\epsilon = [0, 0.0002,.0004,.0006,.0008,.001]$ respectively at $p=1$ across 10 independent trials.

Further, the utility $g(S^\mathcal{A})$ is evaluated at $p \in \{0, \frac{1}{4}, \frac{1}{2}, \frac{3}{4}, 1\}$, averaged over 10 trials for each $\epsilon \in \{0, 0.0002,.0004,.0006,.0008,.001\}$. Notably, the additive noise incurred from the oracle call for $g(S^\mathcal{A})$ accumulates linearly. Specifically, noise of $-\epsilon$ is introduced with probability $p$ in the utility oracle, causing underestimation of $g(S^\mathcal{A})$, which results in more nodes being selected to meet the utility threshold. This leads to an additive increase of $+\epsilon$ in the observed cost $f(S^\mathcal{A})$.

The greedy benchmark $g(\mathcal{GRD})$ represents the noiseless solution. For the MINTSS algorithm, the theoretical bounds are given by $f(\mathcal{GRD}) + \delta\epsilon$ for cost and $g(\mathcal{GRD}) - \delta\epsilon$ for utility, where $\delta = 3 \frac{c_{\max}}{c_{\min}} \ell$ and $\ell = N$ is set based on the maximum oracle calls corresponding to each $\epsilon$ set at $p=1$ and $N=\{22, 23, 27, 39, 39, 39\}$.

% These observations are empirically validated for Cost over $\epsilon$: Figure~1~\hyperref[1a]{(a)} and \hyperref[1b]{(b)},
%     For Utility over $\epsilon$: Figure~1~\hyperref[1c]{(c)} and \hyperref[1d]{(d)}.

% Specifically:
% \begin{itemize}
%     \item Figure~1~\hyperref[1d]{(d)} (utility) and Figure~1~\hyperref[1b]{(b)} (cost) present $g(S^A)$ and $g(\mathcal{GRD})$ across all $p$ values, and $f(S^A)$, $f(\mathcal{GRD})$ respectively too across all $p$ values, illustrating the additive cost effect due to utility underestimation due to noisy oracle calls.
%     \item Figure~1~\hyperref[1c]{(c)} (utility) and Figure~1~\hyperref[1a]{(a)} (cost) present $g(S^A)$ at $p=1$, $g(\mathcal{GRD})$, and $g(\mathcal{GRD}) - \delta\epsilon$, along with the corresponding utility curves and $f(S^A)$ at $p=1$, $f(\mathcal{GRD})$, $f(\mathcal{GRD}) + \delta\epsilon$ corresponding cost curves respectively.
% \end{itemize}
These observations are empirically validated for Submodular Cost Cover Problem for cost over $\epsilon$: Figure~1~\hyperref[1a]{(a)} and \hyperref[1b]{(b)},  
and for Utility over $\epsilon$: Figure~1~\hyperref[1c]{(c)} and \hyperref[1d]{(d)}.

Specifically:
\begin{itemize}
    \item Figure~1~\hyperref[1d]{(d)} (utility) and Figure~1~\hyperref[1b]{(b)} (cost) correspond to the higher relaxation case with $\kappa = 0.98$, $\omega = 0.15$. These plots present $g(S^A)$ across all $p$ values, alongside $g(\mathcal{GRD})$ and the relaxed bound $g(\mathcal{GRD}) - \delta\epsilon$, as well as $f(S^A)$, $f(\mathcal{GRD})$, and $f(\mathcal{GRD}) + \delta\epsilon$. The figures illustrate that despite utility underestimation due to noisy oracle calls, the relaxed constraint allows $S^A$ to remain feasible (i.e., $g(S^A) \leq g(\mathcal{GRD})$), while the utility $f(S^A)$ stays close to $f(\mathcal{GRD})$, capturing the additive cost effect under noise.

    \item Figure~1~\hyperref[1c]{(c)} (utility) and Figure~1~\hyperref[1a]{(a)} (cost) correspond to the lower relaxation case with $\kappa = 0.98$, $\omega = 0.08$. Each figure shows $g(S^A)$ across all $p$ values, $g(\mathcal{GRD})$, and $g(\mathcal{GRD}) - \delta\epsilon$, along with $f(S^A)$, $f(\mathcal{GRD})$, and $f(\mathcal{GRD}) + \delta\epsilon$. In this stricter regime, noise in $g(\cdot)$ leads the algorithm to select an extra element in $S^A$.
\end{itemize}
% \paragraph{Results:}

% \paragraph{Discussion:}



\subsection{Online Bi-Criteria CMAB}
\label{sec:exp:online}

We next evaluate the cumulative regret and constraint violations incurred by the online algorithms our proposed framework. 
In this section, we conduct simulated experiments to evaluate the performance of our proposed algorithm. The primary objectives of the evaluation are as follows:
\begin{enumerate}
\item To demonstrate that the algorithm achieves sublinear \textit{cumulative regret} and \textit{cumulative constraint violation} over time;
\item To analyze the \textit{instantaneous reward} and \textit{instantaneous cost} trajectories, providing insights into the algorithm's real-time decision quality;
\item To study the relationship between \textit{instantaneous utility} and \textit{cumulative regret}, and to illustrate the possibility of achieving negative regret due to constraint-induced improvements in utility.
\end{enumerate}
We begin by describing the experimental setup and implementation details, followed by a detailed analysis of the results.
% \paragraph{Datasets:}

% \paragraph{Baselines:}


\paragraph{Implementation Details:}
\begin{figure}[htbp]
\centering
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/0_r3.png}\\
  \centering \small (a) \label{0a}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/0_r4.png}\\
  \centering \small (b) \label{0b}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/0_r5.png}\\
  \centering \small (c)  \label{0c}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/0_r6.png}\\
  \centering \small (d) \label{0d}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/0_r7.png}\\
  \centering \small (e) \label{0e}
\end{minipage}
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/1_r3.png}\\
  \centering \small (f) \label{1f}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/1_r4.png}\\
  \centering \small (g) \label{1g}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/1_r5.png}\\
  \centering \small (h)  \label{1h}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/1_r6.png}\\
  \centering \small (i) \label{1i}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/1_r7.png}\\
  \centering \small (j) \label{1j}
\end{minipage}
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/2_r3.png}\\
  \centering \small (k) \vspace{0.25em}\\ Cumulative Regret\label{2k}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/2_r4.png}\\
  \centering \small (l) \vspace{0.25em}\\ CCV\label{2l}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/2_r5.png}\\
  \centering \small (m) \vspace{0.25em}\\Instantaneous Utility \label{2m}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/2_r6.png}\\
  \centering \small (n) \vspace{0.25em}\\Instantaneous Cost \label{2n}
\end{minipage}\hfill
\begin{minipage}{0.2\textwidth}
  \includegraphics[width=\linewidth]{Neurips 2025/figures/2_r7.png}\\
  \centering \small (o) \vspace{0.25em}\\ Regret vs Utility\label{2o}
\end{minipage}
\vspace{1em}
\caption{Summary of experimental results across five performance metrics: (a), (f), (k) cumulative regret; (b), (g), (l) cumulative constraint violation (CCV); (c), (h), (m) instantaneous utility; (d), (i), (n) instantaneous cost; and (e), (j), (o) the relationship between instantaneous regret and utility. Each row corresponds to a different value of $\kappa$: the first, second, and third rows correspond to $\kappa = 0.4$, $0.5$, and $0.6$, respectively, with $\omega = 0.1$ fixed across all settings.}
\label{fig:2}
\end{figure}

% \textbf{facebook dataset:}


\subsection{Experiment with Synthetic Data}

We consider a stochastic combinatorial bandit setting with \( n \) arms (influencers), each assigned to exactly one of \( m \) disjoint groups. Let \( h_i \subseteq [n] \) denote the set of arms in group \( i \). The reward at each round \( t \) is defined by a monotone submodular utility function:
\(
g_t(S) = \sum_{i=1}^{m} g_t[i] \cdot \mathbb{1}_{S \cap h_i \neq \emptyset},
\)
where \( w_t[i] \in [0,1] \) denotes the instantaneous utility weight of group \( i \), and \( S \subseteq [n] \) is the set of selected arms. This captures the utility of activating at least one influencer in each group, weighted by group importance at time \( t \).

In addition to utility, we define an additive monotone cost function:
\(
g_t(S) = \sum_{i \in S} c_i,
\)
where \( c_i \in [0,1] \) is the cost associated with pulling arm \( i \). The objective is to select a set \( S \) at each round that minimizes \( g_t(S) \), subject to satisfying the utility constraint \( f_t(S) \geq \kappa - \omega \), where \( \kappa \) is the threshold and \( \omega \) the tolerance.

In our synthetic experiments, the reward function \( f(\texttt{GRD}) \) is constructed so that the offline greedy algorithm achieves the optimal solution \( f(\texttt{OPT}) \). We use this as a benchmark to evaluate the performance of the proposed online algorithm. Specifically, we compare the cumulative cost against the offline optimum and ensure that the utility constraint is satisfied up to a multiplicative \( \beta \)-approximation of \( \kappa \).

\texttt{Implementation details:} We evaluate the proposed approach using synthetic data with \( n = 20 \) base arms, to minimize cost while satisfying the utility threshold \( \kappa \). Experiments are conducted over time horizons \( T \in \{10^4, 10^5, 10^6, 10^7\} \), with each setting repeated for 10 trials. We consider the \emph{weighted cover} reward function and implement an online version of the \texttt{MINTSS} algorithm for Monotone Cost Submodular Cover.

For the \textit{weighted cover} setting, arms are partitioned into \( m = 4 \) groups with sizes \([6, 6, 6, 2]\). At each round \( t \), a stochastic weight vector \( \omega_t \in \mathbb{R}^m \) is sampled with \( \omega_t[i] \sim \text{Unif}([0, i/5]) \) for group \( i \in \{1, 2, 3, 4\} \).

For \( T = 10^7 \), instantaneous performance plots are computed using a sliding window of 100 rounds, averaged over 10 independent trials. We report both the mean and variance of the relevant metrics.

Figures and code are available at the provided link\footnote{\url{https://anonymous.4open.science/r/Online-Bi-Criteria-1503/}}.


\paragraph{Evaluation metrics:}
mention instead of $\alpha T f(\mathrm{OPT})$ using $T f(\mathrm{S^{\mathcal{A}}})$ where $f(\mathrm{S^{\mathcal{A}}})$ is the value of the solution the offline algorithm produces (with access to exact oracles; in practice if we don't have a model for oracle you estimated query values $f(S)$ to high confidence using average of ... Monte Carlo samples.

Also explain penalized regret (we give worst-case regret whenever the constraints are violated); so this provides a fairer view for rewards earned, combining results from constr. viol. with regret % rather than having to 

\paragraph{Results:}
\paragraph{Figure 2-~\hyperref[0a]{(a)}, ~\hyperref[1f]{(f)}, and, ~\hyperref[2k]{(k)} shows the incurred $ \alpha $-regret with respect to $ T $.} For a proxy of $\alpha$ times the optimal, we used the offline algorithm with the mean as the reward, which gives an upper bound on $\alpha$-regret. The regret decreases and eventually reaches a negative value, indicating that the algorithm performs better than $ \alpha $ times the optimal. This behavior is consistent with the upper bounds established in the paper.

\paragraph{Figure 2~\hyperref[0b]{b}, ~\hyperref[1g]{g}, and ~\hyperref[2l]{l} shows the cumulative $ \beta $-constraint violation for different values of $ T $.} On a log-log scale, the straight lines represent a slope of $ 2/3 $. Our cumulative constraint violation (CCV) is lower than this slope, demonstrating the improved performance of the proposed algorithm.

\paragraph{Figures 2-~\hyperref[2c]{c} and 2-~\hyperref[2d]{d} are based on $ T = 10^7 $.}
  Figure 2-~\hyperref[2d]{d} shows that the reward increases over time and stabilizes as arm selections increasingly satisfy the threshold $ \kappa - \omega = 0.4 $ (with $ \kappa = 0.5 $ and $ \omega = 0.1 $).
  Figure 2~~\hyperref[2c]{c} illustrates that the cost stabilizes over time. Together, these figures highlight that the algorithm achieves a low cost while consistently meeting the minimum reward threshold.

 \paragraph{Figure 2~\hyperref[0e]{(e)}, ~\hyperref[1j]{(j)}, and ~\hyperref[2o]{(o)}} This plot illustrates the relationship between instantaneous regret and instantaneous reward. The regret becomes negative when the \texttt{ETCG} algorithm selects sets \( S \) with high marginal gain under the greedy utility function \( f(\texttt{GRD}) \), but violates the utility constraint. As the selected sets begin to satisfy the threshold \( \kappa - \omega \), the instantaneous reward rises, and the algorithm stabilizes on a minimum-cost subset that maintains feasibility. This shift leads the instantaneous regret to return to non-negative values, highlighting the interplay between cost minimization subject to constraint satisfaction.
 

\paragraph{Discussion:}
Figure~2\hyperref[2k]{(k)} shows that at $T = 10^4$, cumulative regret becomes negative. This occurs as the selected subset remains small relative to the feasible set, resulting in lower cost than the greedy solution. Over time, this difference accumulates, leading to negative regret on the log-log scale.

Similarly, Figure~2\hyperref[1g]{(g)} exhibits negative CCV at $T = 10^7$ when the threshold $\kappa - \omega = 0.4$ is satisfied. As seen in Figure~2\hyperref[1h]{(h)}, $f(S^A) > \beta \kappa$ holds early due to high-utility node selection, yielding negative CCV consistent with the derived upper bound.

Figures~2\hyperref[0e]{(e)}, \hyperref[1j]{(j)}, and \hyperref[2o]{(o)} show instantaneous utility versus instantaneous regret. Initially, regret is negative as ETCG selects elements based on marginal gain. The early sets do not meet the utility threshold $\kappa - \omega$, yet satisfy $f(S^A) < \beta f(\text{GRD})$. As selection continues, the utility threshold is reached, but at increased cost, resulting in positive instantaneous cost.

These results correspond to the monotone cost-weighted coverage problem using online MINTSS with $\omega = 0.1$ and varying $\kappa \in \{0.4, 0.5, 0.6\}$ in rows one, two, and three of Figure~\hyperref[fig:2]{2}, respectively.

==> to-do.tex <==
\section{To-dos -- remove at submission}

\todo{minor - Table 1- if time play with column spacing to increase font size more; or maybe bold? to improve readability}

\begin{itemize}
    \item Prior works \shw{
except \cite{crawford2019submodular}
} assumes exact oracles or linear rewards --- maybe mod, MINTSS considered inexact
\end{itemize}

\todo{cjq maybe revise 2.3 to be non-linear obj with bandit?; maybe mention lots of works and we only mention a few, with bandit feedback in 2.3 also we only mention the closest; should cite golovin/streeter and niazadeh for adversarial. }



\todo{minor - better to say 'bi-criteria CMAB' or refer with acronym 'BCCMAB'?}


  \todo{[moved from below Def 1] should we emphasize this (esp. that even if f deterministic, $\epsilon$ error in $g$ evaluation results in additive approximation error for the objective $f$?  
    
    Also, to think about: if g is deterministic and known, (eg like single criteria appx setting in Guanyu's paper) then shouldn't the constraint bound  not have any error term  (up to the $\beta$ term)? would that only be for some algs?  though other way around is different, that even if $f$ deterministic and exact, then error in evaluating $g$ can cause error in the objective function? \red{In MINTSS we have noisy g propagate additive error to deterministic f} <-- but vice versa?}


\todo{[from greedy SCSC] if there's time, skim how Crawford et al articulated challenges in analyzing resilience and mimic for mintss and fairness}


    \todo{[from below Greedy-SCSC] minor - this is like vanilla greedy for max with knapsack constraints, which for that problem has no guarantees unless greedy alg consumes budget fully; double check if have time no issues else maybe add comment (eg if that counterexample has $\gamma=0$}










